A Fast and Accurate One-Stage Approach to Visual Grounding

We propose a simple, fast, and accurate one-stage approach to visual grounding, inspired by the following insight. The performances of existing propose-and-rank two-stage methods are capped by the quality of the region candidates they propose in the first stage --- if none of the candidates could cover the ground truth region, there is no hope in the second stage to rank the right region to the top. To avoid this caveat, we propose a one-stage model that enables end-to-end joint optimization. The main idea is as straightforward as fusing a text query's embedding into the YOLOv3 object detector, augmented by spatial features so as to account for spatial mentions in the query. Despite being simple, this one-stage approach shows great potential in terms of both accuracy and speed for both phrase localization and referring expression comprehension, according to our experiments. Given these results along with careful investigations into some popular region proposals, we advocate for visual grounding a paradigm shift from the conventional two-stage methods to the one-stage framework.

==> related.tex <==
\section{Related Work}
% \zyang{Referring expression comprehension/ phrase localization/ visual grounding/ visual grounding by language queries}
% Visual grounding is the task of 
% Previous two stages-> one stage-> so we...

\noindent {\bf Two-stage visual grounding.}
Visual grounding is the task of localizing the queried region described by a natural language phrase or expression. Most previous studies~\cite{wang2019learning,plummer2017flickr30k,yu2016modeling,mao2016generation} follow a two-stage pipeline. The first stage generates candidate regions with separate region proposal methods~\cite{zitnick2014edge} or pre-trained detectors~\cite{ren2015faster}. The second stage then compute the visual language similarity for each region language pair and `select' the final prediction. A number of studies~\cite{zhang2017discriminative, wang2019learning} model the `select' step as a binary classification task, where each region language pair is tagged with labels `positive', `negative' or `ignored' based on the IoU with the ground-truth queried box. Generating region language triplets and optimize with a maximum-margin ranking loss~\cite{mao2016generation, nagaraja2016modeling, wang2016learning} is another effective approach. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2 or 3 closest current papers:
\noindent {\bf Image-level visual language fusion.}
Several previous studies have explored the idea of image-level visual language fusion on the same or similar tasks. In visual grounding with segmentation output, FCN-style methods~\cite{hu2016segmentation,liu2017recurrent} are proposed to generate pixel-level segmentation masks. Zhao~\textit{et al.} \cite{zhao2018weakly} propose a Multi-scale Anchored Transformer Network (MATN) for weakly supervised phrase localization. The fused image-level visual query feature is used to regress the affine transformation parameters between the box covering the whole image and the predicted queried box. Our study is the most similar to IGOP~\cite{yeh2017interpretable}, which also tries to solve the fully supervised visual grounding task with one-stage frameworks. IGOP encodes image features as a stack of prediction maps by various vision tasks, and generates an energy map based on visual feature maps and the query. The phrase localization task is modeled as finding a box on the energy map that has the smallest energy inside.
Despite the successful exploration on one-stage frameworks, IGOP has two major limitations. First, the use of multiple vision task predictions greatly slow the inference speed. Second, the detached visual features might not capture ideal representation and potentially limit the performance.

